Federated Learning Enables Big Data for Rare Cancer Boundary Detection

Although machine learning (ML) has shown promise in numerous domains, there are concerns about generalizability to out-of-sample data. This is currently addressed by centrally sharing ample, and importantly diverse, data from multiple sites. However, such centralization is challenging to scale (or even not feasible) due to various limitations. Federated ML (FL) provides an alternative to train accurate and generalizable ML models, by only sharing numerical model updates. Here we present findings from the largest FL study to-date, involving data from 71 healthcare institutions across 6 continents, to generate an automatic tumor boundary detector for the rare disease of glioblastoma, utilizing the largest dataset of such patients ever used in the literature (25,256 MRI scans from 6,314 patients). We demonstrate a 33% improvement over a publicly trained model to delineate the surgically targetable tumor, and 23% improvement over the tumor's entire extent. We anticipate our study to: 1) enable more studies in healthcare informed by large and diverse data, ensuring meaningful results for rare diseases and underrepresented populations, 2) facilitate further quantitative analyses for glioblastoma via performance optimization of our consensus model for eventual public release, and 3) demonstrate the effectiveness of FL at such scale and task complexity as a paradigm shift for multi-site collaborations, alleviating the need for data sharing.

==> CollaboratorSummary.tex <==
% Short Summary of collaborator and no of cases

=======================================================
Total sites in the study:71

No of sites participated in Full federation(excluding OldBraTS and TCIA):49
No of sites from TCIA:13
No of sites from Old BraTS: 3
no of sites for Validation Only:6 

=======================================================
Total Cases for FeTS study: 6314
Total cases to train PIM: 231
Total Cases For Validation only sites: 590
Total cases excluding PIM = 6083
Total cases excluding PIM and Validation only sites: 5493
=======================================================

No of sites for preliminary federation including OldBraTS and TCIA:35
Total cases for preliminary federation: 2471
Site IDs: 2,3,9,14,22,23,24,27,28,29,31,33,36,37,41,46,53,54,59
% NEED TO DISCUSS ABOUT IOWA

=======================================================

Details for PIM:
Old BraTS cases from 3 sites: 23
TCIA cases from 13 sites: 208
Total sites for PIM: 13+3 = 16
Total PIM cases: 208+23=231
PIM site IDs: 47,51,55,57,58,61,62,63,64,65,66,67,68,69,70,71

========================================================

Number of cases for validation only sites:
MOffitt:100
ACR:112
Colorado:100
Leeds: 120
KCL: 58
Queesn: 100
Total cases: 100+112+100+120+58+100 = 590

========================================================
%First/Middle/Last name of authors with orcid+email id is in  collaborator master
%-->Final_Co-authors_Nature_S1 sheet

==> cover_letter.tex <==
- "true" federation would be time-consuming to set up, and we are happy to set this up, subject to the collaborators' ability (in terms of availability of their time and hardware)





Following your positive response on our presubmission enquiry, we are submitting our work entitled “Federated Learning Enables Big Data for Rare Cancer Boundary Detection” for review in Nature.

Although machine learning has shown promise in numerous domains, there are concerns about reproducibility and generalization to out-of-sample data. Particularly, since multi-institutional collaborations are challenging to reach a global scale to generate sufficiently diverse centralized datasets, due to various technical, cultural, privacy, and regulatory limitations. This is particularly important in domains such as healthcare, where accumulation of large and importantly diverse datasets is essential to address health disparities, under-served populations, and even rare diseases. This has recently even been recognized by governmental agencies, such as the National Institutes of Health (NIH) of the United States, which created a special funding program named “Artificial Intelligence/Machine Learning Consortium to Advance Health Equity and Researcher Diversity (AIM-AHEAD)” to leverage federated learning for developing machine learning models on healthcare data towards addressing health disparities and inequities.

In this work, we report on the largest real-world federation to-date, involving data from 71 healthcare institutions across 6 continents, to generate an automatic cancer boundary detector, utilizing the largest dataset of glioblastoma patients ever used in the literature (n=6,314), while all the data were always retained within the acquiring institutions. It is the use of federated learning that enabled all these institutions to participate in this collaborative network, attempting to develop a model gaining knowledge from such an unprecedented dataset. To the best of our knowledge, this is the largest dataset ever considered for this rare cancer. We would like to emphasize that even though we used glioblastoma as a case example in this study, the approach of federated learning used here is very general and applicable to any domain – we are already aware of use cases using the federated learning framework used in this study (i.e., OpenFL) in the financial sector, as well as on assessing vital signals of astronauts. We anticipate that federated learning will become the default mechanism of conducting machine learning research while preserving data silos. This would hopefully ensure that models trained using federated learning would be far more widely applicable compared to those trained using data from a handful of sites.

Taking all the above into consideration, as well as the scope of your journal, we would greatly appreciate it if you would consider the review of this manuscript, as we strongly believe that release of the manuscript and the associated trained consensus models and source code will be of broad interest in the readership of Nature. We confirm that this work is original and has not been published elsewhere nor is it currently under consideration for publication elsewhere.

Please do not hesitate to contact me if you need any further information.

Thank you for taking the time to consider our enquiry, and I look forward to your response.





The senior and corresponding author of this manuscript has been interacting with the Senior Editor (Dr. Victoria Aranda) through email discussions about this real-world study, as well as a previous simulated study (now published in Sci Rep), being considered for review in Nature. The last communication resulted in a formal presubmission enquiry (ID: 2022-01-01128). The editor has responded positively on considering the manuscript for publication, following its successful review.






*Nature offers a transparent peer review option for new original research manuscripts submitted from 1st December 2019. We encourage increased transparency in peer review by publishing the reviewer comments and the authors’ rebuttal letters of published articles, if the authors agree. This material is made available as a supplementary peer review file under an Open Access Creative Commons CC -BY License. If you wish to opt in to transparent peer review please provide your response to reviewers as a .doc file where possible.

Please note we allow redactions to authors’ rebuttal and reviewer comments in the interest of confidentiality. If you are concerned about the release of confidential data, let us know specifically what information you would like to have removed. We cannot incorporate redactions for any other reasons. Reviewer names will be published in the peer review file if the reviewers have signed their comments to authors, or they explicitly agree to release their name. For more information, please refer to our FAQ page.

Note that this initiative applies only to original research articles that are published. All editorial decisions and processes are independent of your decision to participate in transparent peer review. You will be able to change your selection at each round of revision; if you are submitting the final version of the manuscript, we will consider your choice final. There may be cases when Springer Nature cannot publish peer reviews or rebuttals and we reserve the right to withhold transparent peer review.

Yes, I do want to participate in transparent peer review
No, I do not want to participate in transparent peer review

==> of no use/0_skeleton.tex <==
\begin{enumerate}
    \item All collaborators should be blinded, and the final indexing information should be present in appendix
    \item \textbf{Intro}
        \begin{enumerate}
            \item Healthcare-Data-AI
            \item Federated Learning as a paradigm shift
            \item Simulated studies (refer to the 4 findings of our Sci Rep paper, and others)
            \item Real-world examples (refer to the 2-3 cases of individual 5-collab papers)
            \item Our study addresses ...
        \end{enumerate}
    \item \textbf{Results/Findings}%: each "result" goes as a "finding": plots: https://github.com/FETS-AI/supremacy_paper_stats/blob/main/BaseTableGeneration.ipynb
        \begin{enumerate}
            \item Adding diverse data improves performance
            \item Evaluation of consensus model(s) across each collaborator. (diagonal table/matrix figure - though in Nature Reports paper we had individual institution models to compare against, here we will only have the initial publicly trained model to compare against)
            \item Ample and Diverse Data can Mitigate the Need for Unreasonable Computational Resources for a Clinical Environment, i.e., Lead to More Translatable Models (our single ResUNet vs DeepScan vs nnUNet) - possibly sub-Findings too for each picking on large RAM and engineering solution
            \item Stable convergence curves is observed ONLY on collabs with reasonably large data (check on graphs)
            \item Large regions show better results (WT is better than TC - TC is better than ET (check on graphs)): show number of collaborators where WT is on top, TC is on top and ET is on top
            \item Best model with "average" score across all regions v/s models with best scores across each region (ET, TC, WT)
            \begin{enumerate}
                \item ModelVersion 24:
                    \begin{itemize}
                        \item float\_DICE\_WT: 0.88878
                        \item binary\_DICE\_WT: 0.891048
                        \item binary\_Hausdorff95\_TC: 12.917994
                        \item binary\_Hausdorff95\_WT: 5.870099
                        \item binary\_Sensitivity\_TC: 0.863264
                        \item binary\_Sensitivity\_WT: 0.911302
                        \item MeanBinaryHausdorff: 13.722721
                    \end{itemize}
                \item ModelVersion 40:
                    \begin{itemize}
                        \item float\_DICE\_ET: 0.788595
                        \item float\_DICE\_TC: 0.818254
                        \item binary\_DICE\_TC: 0.829001
                        \item MeanBinaryDICE: 0.839396
                    \end{itemize}
                \item ModelVersion 69:
                    \begin{itemize}
                        \item binary\_DICE\_ET
                        \item binary\_Specificity\_ET
                        \item binary\_Specificity\_TC: 0.999772
                    \end{itemize}
                \item ModelVersion 30:
                    \begin{itemize}
                        \item binary\_Sensitivity\_ET: 0.883931
                    \end{itemize}
                \item ModelVersion 42:
                    \begin{itemize}
                        \item binary\_Hausdorff95\_ET: 20.890074
                    \end{itemize}
                \item ModelVersion 67:
                    \begin{itemize}
                        \item binary\_Specificity\_WT: 0.999432
                    \end{itemize}
            \end{enumerate}
            \item FeTS consensus model vs BraTS best model (nnUNet) - The answer is in the data
            \item Best model per collaborator vs best consensus model
            \item Locally updated models vs consensus models
            \item Unseen validation data results
            \begin{itemize}
                \item comparison with nnunet would (most likely) result in nnunet performing better, which is likely because nnunet was used in ground truth creation
                \item if the ground truth was created using a method that under-segmented and allowed annotators to delineate the boundary regions, the final GT would be closer to "gold standard"
                \item for ideal gold standard GT creation, multiple annotators should delineate the boundaries of the regions of interest and a majority voting done for each voxel under consideration
            \end{itemize}
            \item Validation participation dropouts (figs shown by Hans on 2021/Aug/09)
            \begin{enumerate}
                \item dropout does not affect model performance a lot
                \item missing data during dropout doesn't seem to have noticeable impact
                \item effect of interpolation for the missing rounds
            \end{enumerate}
            \item Appropriate coordination is essential (curation/preprocessing)
            \item Maybe something from questionnaire 
        \end{enumerate}
    \item \textbf{Discussion}
        \begin{enumerate}
            \item We have shown that ...
            \item Our Previous Simulated Findings
                \begin{enumerate}
                    \item Ample and diverse data are needed
                    \item Collaborative learning is superior
                    \item FL performs comparably to data-sharing
                    \item Model learning during FL is more stable than during incremental methods
                \end{enumerate}
            \item FeTS development - Formulation of FeTS initiative
            \item Data Discovery and Curation
            \item Establishing the Harmonized Preprocessing
            \item Data quality will determine the real world application
                \begin{enumerate}
                    \item Model collapse during early trial run
                    \item Filtering updates
                    \item Data quality sanity checks
                \end{enumerate}
            \item Establishing Evaluation Framework
            \item Discussion on Results
            \item segmentation is a difficult problem, especially with FL
            \item Model selection and dropout
                \begin{enumerate}
                    \item We see a trend of "higher-dropout = better score". Could be catastrophic forgetting (dropouts return, consensus model has forgotten them, they yield worse scores). Could be harder data, e.g. an institution with less compute/network/participation capacity might also have less data curation capacity, such that "difficulty" is more about data quality than actual patient trends.
                \end{enumerate}
            \item The current model was trained on a Dice loss. Future studies could focus on a combination of different metrics, specifically the ones used for validation, to be used as the training loss
            \item Privacy and Security for Healthcare
            \item Concluding Remarks
        \end{enumerate}
    \item \textbf{Supplementary}
        \begin{enumerate}
            \item Methods
            \item Data
            \item Evaluation Framework
        \end{enumerate}
\end{enumerate}

==> of no use/4_discussion.tex <==
\subsection{Governing a federation}

    A significant amount of coordination took place to set up a real-world multi-national federation, and the effort of the current study provided a good deal of experience as to what the pain points can be in this process. As FeTS/OpenFL governance was still maturing at the time we initiated the effort, much of this work was manual for us. The coordination began with resource gathering at the various sites in the form of site technical leads and site compute resources. With the technical leads, we then proceeded to perform tests of the workload to further identify gaps in the requirements (network configurations, data center requirements, etc). We then proceeded with data curation and pre-processing, and finally connected individual sites to the FL aggregator to start their participation.

    Ensuring that the annotation protocol is followed is vital for the model to learn correct information, and a good deal of automated validation of this pipeline was helpful in identifying issues.

    In general, debugging data is more difficult during federated learning due to the coordination and or privacy issues involved. We gained a good deal of experience during this effort that went into further development of data sanity checking tools included in the FeTS code base. We look forward to continued work towards general solutions in this space.

%\subsection{Re-defining ``ground truth'' annotation}
%Comparison of the final consensus model with nnU-Net against the out-of-sample dataset results in the latter performing better. This is presumably because nnU-Net was used to inform ground truth (GT) creation at some sites (see Section.~\ref{methods:data} for details)
%If the preliminary GT annotation was created using a method that under-segmented the tumor regions, thus allowing annotators (i.e., clinical experts) to delineate the boundary regions with manual corrections, the final GT would be closer to a ``gold standard''. For ideal gold standard GT creation, multiple annotators (i.e., clinical experts) should delineate the boundaries of the regions of interest and a majority voting be performed for each voxel under consideration.
%\iffalse
%Would a mention of annotation reproducibility or stability \cite{pati2020reproducibility} make sense here?
%\fi

\subsection{Open-sourcing the final models}
    In the spirit of Findability, Accessibility, Interoperability, and Reusability (FAIR) \cite{wilkinson2016fair} in open science, we have open-sourced the final \textit{singlet} and \textit{triplet} consensus models (see Section.~\ref{findings:singlet_triplet} for details), including the complete source-code used in the project.


A few sentences on limitations of the current study

A closing paragraph of conclusions, context, and future outlook.

\fxfatal{For group discussion: licensing terms for the models, say more about importance of open source above and how other studies have not gone that direction?}
    
    
    


==> of no use/5_todo.tex <==
%SB: Ujjwal doing the table for inst contributions
%   Spyros is working on the description

% Contact all by Wednesday
%                       for dates, timeline, orcid, demographics


% Personalization finding : check with Brandon

% Collaborators feedback based on survey - table in manuscript is current.

% Here are the word counts per section 2022/02/01:
% Abstract: 294
% Introduction: 1064
% Findings: 2582
% Discussion: 363
% Methods: 3613



%Email to collaborators:
% we need demographics (table in Google docs)


%To discuss
    % demographics table
    % contributions
% Experiments on centralized out of sample : ACR?


(Our work is done, KCL, Mofitt, Leeds, Colorado are done, ACR remains as of 2021/10/13) Pick which models to score on unseen out-of-distribution data (i.e., from sites that were not involved in the training phase):
    1. (IL) Pick 10-30 model triplets we want to score on these unseen data.
        Include the initial model (trained on public BraTS 2020 data).
    2. (Sarthak) Set up installer to use all 30 models.

(Not Needed? - we are interpolating to obtain missing validation scores when needed)Fill in missing validation scores:
    1. (IL) Modify existing validation script to allow validation data only, and to score multiple models; integrate into validation executable. 
    2. (IL) Identify exactly which models to score
        - [TODO] identify which "best" models we have scored that contain "gaps" during the validation step of the training (and which exact sites), and see if these can be re-run for the collaborators that did not contribute for that round
    3. (IL) Identify exactly which collaborators to request scores from
    4. (Sarthak) Contact collaborators to see which still have data available and can help
    
Get single institution model comparisons (against consensus models).
    1. (Joint) Come up with argument for the minimum size required to be a 'viable' single institution model, then identify which institutions have this much data. Proposal? (double than the minimum requested amount, i.e., 200 cases at least)
    
    Here is the data - The ones with greater than 200 data samples are: nradheidelberg, DellSP, escalabr, and FQDN. Dropping to 150 only gets us an additional uwisc and LenovoP720, and dropping to 100 gives a total of 35 institutions.
        - 2021/10/14: umang (symbiosis) is ready to train
        - [TODO] Sarthak to reach out to Umang to check - if he can do it, then Spyros/Sarthak will check with HBerg and Evan; we have data for the rest
    2. (Joint) Train single institution models for those identified above.
    3. (Sarthak?)Send above models to unseen out-of-distribution data owners in order to obtaining test scores against these models.
    4. Ensemble single site models (of these 4-5 sites) and compare with consensus and single models.
    
Understand terrible WT scores:
    1. (IL) Identify collaborators with low WT scores (TUM, Zurich, UPenn, Iowa/RadOncMaps)
        - [TODO] perhaps identify collaborators with low scores for WT/TC/ET; Only representative examples (no need for completeness) need to have a threshold for the collaborators with a specific number of cases (perhaps 100?)
    2. (IL) Ensure computations are correct
    3. (Sarthak) Reach to collaborators with verified bad WT scores to look at data
    
    - SP: check with the point of contact to check if the previous logs of the run is present or noticed
    - iowa: check with choi and if they have all the data, SB will follow up with Baek
        - 2021/10/19: SP emailed J.Choi
    - concepcion
        - 2021/10/19: UB emailed
    - henry ford (we have it, they just need to send us the val.csv)
        - 2021/10/19: SP emailed L.Bing
    - georgetown (we have it)



    1. (Spyros) Identify collaborator with exceptionally good scores beyond glioma (UPatras)
        - identify example case(s)
        - run the consensus model to report on the perf of the final model too.
        

==> of no use/DISCUSSION_draft_notes.tex <==
\iffalse
\subsection{Getting a federation off the ground}
    \begin{itemize}
        \item Significant amount of coordination is required during data curation and preprocessing steps
        \item Ensuring annotation protocol is followed is vital for the model to learn correct information
    \end{itemize}
\subsection{Limitations of this model}
    \begin{itemize}
        \item The consensus model does not run on every code base, and needs a dedicated software architecture
        \item Initiatives such as MedPerf \cite{karargyris2021medperf} would be good to enable usage of this consensus model on different FL back-ends
    \end{itemize}
\subsection{Re-defining ``ground truth'' annotation}
    \begin{itemize}
        \item comparison of the final consensus with nnU-Net with the out-of-sample dataset results in the latter performing marginally better, which is because nnU-Net was used in ground truth creation (see Section.~\ref{methods:data} for details)
        \item if the ground truth was created using a method that under-segmented and allowed annotators (i.e., clinical experts) to delineate the boundary regions, the final GT would be closer to a ``gold standard''.
        \item for ideal gold standard GT creation, multiple annotators (i.e., clinical experts) should delineate the boundaries of the regions of interest and a majority voting done for each voxel under consideration.
    \end{itemize}
\subsection{Open-sourcing the final models}
    \begin{itemize}
        \item In the spirit of Findability, Accessibility, Interoperability, and Reusability (FAIR) \cite{wilkinson2016fair} in open science, we have open-sourced the final singlet and triplet consensus models (see Section.~\ref{findings:singlet_triplet} for details), including the complete source-code used in the project.
        \item Perhaps a less subtle jab at ``other'' FL studies that do not make their code and models publicly available?
        \item \fxfatal{For group discussion: licensing terms for the models}
    \end{itemize}
\fi

==> of no use/FIGURE_LEGENDS.tex <==
\section*{Figure Legends}

\begin{itemize}
    \item \textbf{Figure~\ref{fig:map}.} Representation of the study's global scale, diversity, and complexity. \textbf{a}, The map of all sites involved in the development of FL consensus model. \textbf{b}, example of a GBM mpMRI scan with corresponding reference annotations of the tumor sub-compartments. \textbf{c-d}, comparative performance evaluation of the final consensus model with the public initial model on the collaborators' local validation data (in \textbf{c}) and on the complete out-of-sample data (in \textbf{d}), per tumor sub-compartment. Note the box and whiskers inside each violin plot, represent the true min and max values. The top and bottom of each ``box'' depict the 3rd and 1st quartile of each measure. The white line and the red $\times$, within each box, indicate the median and mean values, respectively. The fact that these are not necessarily at the centre of each box indicates the skewness of the distribution over different cases. The ``whiskers'' drawn above and below each box depict the extremal observations still within $1.5$ times the interquartile range, above the 3rd or below the 1st quartile. \textbf{e}, number of contributed cases per collaborating site.
    \item \textbf{Figure~\ref{fig:benefits_of_fl}.} Generalizability evaluation on `centralized' out-of-sample data, per tumor sub-compartment and averaged across cases. Comparative performance evaluation across the public initial model, the preliminary consensus model, the final consensus model, and an ensemble of single site models from collaborators holding $>200$ samples.
    \item \textbf{Figure~\ref{fig:dice_across_regions}.} Global consensus model validation curves. \textbf{a}, of participating sites across training rounds showing that the score is greater for sub-compartments with larger volumes. \textbf{b}, for all considered sub-compartments, of a site with problematic annotations (Site 48). The instability in these curves could be caused by errors in annotation for the local validation data (similar to errors that were observed for a small shared sample of data from this site).  Shading indicates 95\% confidence intervals over cases. \textbf{c}, an example of a case with erroneous annotations in the data used by Site 48.
    %\item \textbf{Figure~\ref{fig:fed_col_counts}.} Collaborator full data size histogram for the institutions performing. \textbf{a}, preliminary versus full federation. \textbf{b}, single institution training versus those in the full federation.
\end{itemize}



\section*{Extended Figure Legends}

\begin{itemize}
    \item \textbf{Figure~\ref{fig:fl_approaches}.} Illustration of the different approaches to train DL models during multi-site collaborations. \textbf{a}, Institutional incremental learning (IIL). \textbf{b}, Cyclic Institutional incremental learning. \textbf{c}, Federated learning by independent aggregation. \textbf{d}, Centralized learning by aggregating data.
    \item \textbf{Figure~\ref{fig:unet}.} Illustration of the U-Net architecture with residual connections, plotted using PlotNeuralNet \url{https://github.com/HarisIqbal88/PlotNeuralNet}. One spatial dimension is left out for clarity.
    \item \textbf{Figure~\ref{fig:single_and_consensus_models_against_holdout_singles}.} Comparative performance evaluation of the final consensus model, per tumor sub-compartment and averaged across cases. Comparison with the public initial model with each single site model (for collaborators holding $>200$ samples), as well as with their ensemble. Significance of results (Wilcoxon signed-rank test): Site 1: $p_{Average}=2\times 10^{-7}$, $p_{ET}=4\times 10^{-8}$, $p_{TC}=6\times 10^{-8}$, $p_{WT}=2\times 10^{-9}$; Site 2: $p_{Average}=5\times 10^{-6}$, $p_{ET}=1\times 10^{-5}$, $p_{TC}=1\times 10^{-4}$, $p_{WT}=1\times 10^{-4}$, Site 3: $p_{Average}=3\times 10^{-7}$, $p_{ET}=2\times 10^{-6}$, $p_{TC}=1\times 10^{-6}$, $p_{WT}=6\times 10^{-9}$, Site 4: $p_{Average}=4\times 10^{-6}$, $p_{ET}=5\times 10^{-5}$, $p_{TC}=8\times 10^{-7}$, $p_{WT}=8\times 10^{-3}$. 
\end{itemize}


==> of no use/FINDINGS_draft_notes.tex <==
%This file includes material that sat in the main results file, for sanity checking prior to word pruning

\iffalse
        \begin{enumerate}
            \item Adding diverse data improves performance
            \item Evaluation of consensus model(s) across each collaborator. 
            
            \item Ample and Diverse Data can Mitigate the Need for Unreasonable Computational Resources for a Clinical Environment, i.e., Lead to More Translatable Models (our single ResUNet vs DeepScan vs nnUNet) - possibly sub-Findings too for each picking on large RAM and engineering solution
            \item Stable convergence curves is observed ONLY on collabs with reasonably large data (check on graphs)
            \item Large regions show better results (WT is better than TC - TC is better than ET (check on graphs)): show number of collaborators where WT is on top, TC is on top and ET is on top
            \item Best model with "average" score across all regions v/s models with best scores across each region (ET, TC, WT)
            \begin{enumerate}
                \item ModelVersion 24:
                    \begin{itemize}
                        \item float\_DICE\_WT: 0.88878
                        \item binary\_DICE\_WT: 0.891048
                        \item binary\_Hausdorff95\_TC: 12.917994
                        \item binary\_Hausdorff95\_WT: 5.870099
                        \item binary\_Sensitivity\_TC: 0.863264
                        \item binary\_Sensitivity\_WT: 0.911302
                        \item MeanBinaryHausdorff: 13.722721
                    \end{itemize}
                \item ModelVersion 40:
                    \begin{itemize}
                        \item float\_DICE\_ET: 0.788595
                        \item float\_DICE\_TC: 0.818254
                        \item binary\_DICE\_TC: 0.829001
                        \item MeanBinaryDICE: 0.839396
                    \end{itemize}
                \item ModelVersion 69:
                    \begin{itemize}
                        \item binary\_DICE\_ET
                        \item binary\_Specificity\_ET
                        \item binary\_Specificity\_TC: 0.999772
                    \end{itemize}
                \item ModelVersion 30:
                    \begin{itemize}
                        \item binary\_Sensitivity\_ET: 0.883931
                    \end{itemize}
                \item ModelVersion 42:
                    \begin{itemize}
                        \item binary\_Hausdorff95\_ET: 20.890074
                    \end{itemize}
                \item ModelVersion 67:
                    \begin{itemize}
                        \item binary\_Specificity\_WT: 0.999432
                    \end{itemize}
            \end{enumerate}
            \item FeTS consensus model vs BraTS best model (nnUNet) - The answer is in the data
            \item Best model per collaborator vs best consensus model
            \item Locally updated models vs consensus models
            \item Unseen validation data results
            \begin{itemize}
                \item comparison with nnunet would (most likely) result in nnunet performing better, which is likely because nnunet was used in ground truth creation
                \item if the ground truth was created using a method that under-segmented and allowed annotators to delineate the boundary regions, the final GT would be closer to "gold standard"
                \item for ideal gold standard GT creation, multiple annotators should delineate the boundaries of the regions of interest and a majority voting done for each voxel under consideration
            \end{itemize}
            \item Validation participation dropouts (figs shown by Hans on 2021/Aug/09)
            \begin{enumerate}
                \item dropout does not affect model performance a lot
                \item missing data during dropout doesn't seem to have noticeable impact
                \item effect of interpolation for the missing rounds
            \end{enumerate}
            \item Appropriate coordination is essential (curation/preprocessing)
            \item Maybe something from questionnaire 
        \end{enumerate}
        
        
\subsection{Convergence Curve Stability is (will talk about this in intro based on our Nat Sci paper)}
    \fxnote{Might talk about this during introduction, by referring Sheller Nat Sci paper}
    \begin{itemize}
        \item We do not find a strong correlation between dropping out and instability of the convergence curve (will provide figure here).
        \item There is no apparent correlation between convergence curve stability and the size of the training data (see Fig.~\ref{conv_stability_over_size}).
        \item Provide formal definition for the stability measure being used here: If a validation curve is given by \textbf{x}, \textbf{y} where $\textbf{x}=\langle x_{1}, ..., x_{n}\rangle$ is an array of rounds and $\textbf{y}=\langle y_{1}, ..., y_{n}\rangle$ is the associated array of validation scores, our validation curve stability measures the variation in $\textbf{y}$, disregarding potentially irregular spacing in the round values due to missing validation scores. Specifically, the stability is computed as: $\sum_{i=2}^{i=n}{|y_i - y_{i-1}|}$. Note that though validation curves are displayed in this work with confidence intervals computed over individual case validation results, we compute curve stability using the curve of the mean values over cases.  
        \begin{figure}
          \centering
          \includegraphics[width=0.5\textwidth]{figures/stability_vs_data_size.png}
          \caption{Stability of the validation curve by institution validation set size.}
          \label{conv_stability_over_size}
       \end{figure}
    \end{itemize}
    
    \begin{itemize}
        \item Four collaborators with most stable convergence curves and at least 5 validation samples (See Fig.~\ref{four_stable_curves}).
        \begin{figure}
          \centering
          \includegraphics[width=0.4\textwidth]{figures/institution_8_convergence_curve.png}
          \includegraphics[width=0.4\textwidth]{figures/institution_20_convergence_curve.png}
          \includegraphics[width=0.4\textwidth]{figures/institution_50_convergence_curve.png}
          \includegraphics[width=0.4\textwidth]{figures/institution_38_convergence_curve.png}
          \caption{Four collaborators with the most stable learning curves among collaborators holding more than 5 validation samples.}
          \label{four_stable_curves}
       \end{figure}
        \item Four collaborators with least stable convergence curves with more than 50 samples and not low validation scores (See Fig.~\ref{four_unstable_curves}).
        \begin{figure}
          \centering
          \includegraphics[width=0.4\textwidth]{figures/institution_7_convergence_curve.png}
          \includegraphics[width=0.4\textwidth]{figures/institution_11_convergence_curve.png}
          \includegraphics[width=0.4\textwidth]{figures/institution_9_convergence_curve.png}
          \includegraphics[width=0.4\textwidth]{figures/institution_51_convergence_curve.png}
          \caption{Four collaborators with the least stable learning curves among collaborators holding more than 5 validation samples.}
          \label{four_unstable_curves}
       \end{figure}
        \item try and draw inferences from this
    \end{itemize}
    
\subsection{Validation participation disconnects (BE: not sure if we keep this, the only result I think we have here is the saw-tooth example referred to above)}
    % can go in discussion or supplementary
    %\fxfatal{use figs shown by Hans on 2021/Aug/09}
    \begin{itemize}
        \item Effect of disconnect towards model performance
        \item Effect of missing data towards convergence curve
        \item Disconnect does not affect model performance a lot
        \item missing data during disconnect doesn't seem to have noticeable impact
        \item Effect of interpolation for the missing rounds
    \end{itemize}
\fi
    
%% micah comment: do we need to caveat this a little bit given that the ensemble performs very close to the consensus model on the two holdout sets? We definitely show this, but we also have an open question that needs future study to understand the ensemble vs. consensus performance. We may find in the future that poor quality data does more harm than good. 


\subsection*{More data can improve performance}
   
    % had said 'using n=273 cases' below, but the initial training used a total of 231 cases split into train/val. 
    

    \iffalse
    \begin{itemize}
        \item Model trained on publicly available data performs with an average \textit{DICE} score of 0.66 across all 3 regions for all collaborators
        \item Once more data is introduced and a final consensus model (model from round 52) is selected to maximize the mean binary \textit{DICE} over all three regions (interpolating to fill in missing validating institutions), the trained model gains performance improvement of $27\%$ for ET, $33\%$ for TC, and $16\%$ for WT. Here the comparison is performed using only the institutions who validated during round 52 so that both initial and consensus model validation scores exist (See Fig.~\ref{benefits_of_fed} %- also see  \ref{phase1_benefits_of_fed} for the benefits during the first phase of training and 
        - also see Fig.~\ref{fig:benefits_of_fed_by_size} for per institution increases from initial model scores to individually selected consensus models per institution by validation set size)
        \item Using held-out data collected at institutions independent from those used in federation, we see an incremental improvement over the public initial model for the ET and TC segmentation tasks when going from a consensus model resulting from federated training with a subset of institutions compared to the consensus model resulting from a federation with all institutions. For the ET task the improvement over the public initial model goes from $14\%$ to $19\%$, and for TC segmentation the improvement goes from $23\%$ to $28\%$. (see Fig.~\ref{fig:prelim_and_full_consensus_and_initial_against_holdout})
        \item Federated consensus models are superior to ensemble of subset of single institutions models for the ET and TC segmentation tasks (See Fig.~\ref{fig:single_and_consensus_models_against_holdout}). 
    \end{itemize}
    \fi
    
    \iffalse
    \begin{figure}
      \centering
      \includegraphics[width=0.9\textwidth]{figures/performance_increase_restricted_init_boxplots.png}
      \caption{Validation data \textit{DICE} scores for the public initial model and federated consensus model (per region of interest) along with percent increases of the mean over cases of the consensus model \textit{DICE} compared to the initial model.}
      \label{fig:benefits_of_fed}
    \end{figure}
    
    \begin{figure}
      \centering
      \includegraphics[width=0.9\textwidth]{figures/init_scores_versus_consensus_against_holdout.png}
      \caption{Out-of-sample data \textit{DICE} scores for the public initial model and federated consensus model (per region of interest) along with percent increases of the mean over cases of the consensus model \textit{DICE} compared to the initial model.}
      \label{fig:benefits_of_fed_against_out_of_sample}
    \end{figure}
\fi
    
    \iffalse
    \begin{figure}
        \centering
        \includegraphics[width=0.9\textwidth]{figures/percent_increase_inst_by_val_set_size.png}
        \caption{Percentage increase in mean \textit{DICE} of best model (by validation score) seen at each institution over their validation of the public initial model (by institution validation set size). One data point is not included. Institution 6 scored the initial model using a single validation sample with a mean \textit{DICE} score of 1.07e-10. The corresponding consensus model score for this institution was 0.788, representing an increase of over 700 billion percent.}
        \label{fig:benefits_of_fed_by_size}
        \fxwarning{SP: we should probably not put this figure in, doesn't fit with the narrative}
    \end{figure}
    \fi

  %  \begin{figure}
  %    \centering
  %    \includegraphics[width=0.9\textwidth]{figures/phase1_performance_increase_full_init.png}
  %    \caption{Percentage increase of consensus model \textit{DICE} score overpublic initial model (per region of interest) for the first phase of training with 28 training institutions.}
  %    \label{phase1_benefits_of_fed}
  %  \end{figure}
  
  
      % SP on 2022/01/31: as per the formatting guide, a ‘modest’ display item is one that, with its legend, occupies about a quarter of a page (equivalent to ~270 words)
    \iffalse
    \begin{figure}
        \centering
        \begin{subfigure}[t]{0.03\textwidth}
        \textbf{a}
        \end{subfigure}
        \begin{subfigure}[t]{0.44\textwidth}
            %\centering
            \includegraphics[width=\textwidth]{figures/prelim_and_full_consens_and_initial_against_holdout_reg_scale.png}
        \end{subfigure}
        \hfill
        \begin{subfigure}[t]{0.03\textwidth}
        \textbf{b}
        \end{subfigure}
        \begin{subfigure}[t]{0.44\textwidth}
            %\centering
            \includegraphics[width=\textwidth]{figures/single_and_consensus_models_against_holdout.png}
        \end{subfigure}
        \caption{Performance evaluation of final consensus model on centralized out-of-sample data, per tumor sub-compartment and averaged across. \textbf{a}, comparative assessment with the initial and with the preliminary smaller federation consensus models (Section~\ref{methods:federation}). \textbf{b}, comparative assessment with each single institution model (for the subset of collaborators holding more than 150 samples), as well as with their ensemble.}
        \label{fig:benefits_of_fl_single}
        \label{fig:prelim_and_full_consensus_and_initial_against_holdout_reg_scale}
        \label{fig:single_and_consensus_models_against_holdout}
    \end{figure}
    \fi

    \begin{figure}
        \centering
        \begin{subfigure}[t]{0.03\textwidth}
        \textbf{a}
        \end{subfigure}
        \begin{subfigure}[t]{0.44\textwidth}
            %\centering
            \includegraphics[width=\textwidth, valign=t]{figures/prelim_and_full_consens_and_initial_against_holdout_reg_scale.png}
            \label{fig:prelim_and_full_consensus_and_initial_against_holdout_reg_scale}
        \end{subfigure}
        \hfill
        \begin{subfigure}[t]{0.03\textwidth}
        \textbf{b}
        \end{subfigure}
        \begin{subfigure}[t]{0.44\textwidth}
            %\centering
            \includegraphics[width=\textwidth, valign=t]{figures/single_and_consensus_models_against_holdout.png}
            \label{fig:single_and_consensus_models_against_holdout}
        \end{subfigure}
        \caption{Performance evaluation of final consensus model on centralized out-of-sample data, per tumor sub-compartment and averaged across. \textbf{a}, comparative assessment with the initial and with the preliminary smaller federation consensus models (Section~\ref{methods:federation}). \textbf{b}, comparative assessment with each single institution model (for the subset of collaborators holding more than 150 samples), as well as with their ensemble.}
        \label{fig:benefits_of_fl_single}
    \end{figure}
    
    
    \subsection*{FL is robust to some annotation errors}

    \iffalse
    \subsection{Baseline FedAvg is robust to some annotation errors, but not all}
        \begin{itemize}
            \item Institution with blank images led to NANs in updates, which destroyed model
            \item Correct solution is future research: the training error called our attention, allowing us to fix issue
            \item Institution with incorrect label schema failed to learn well, implying minimal impact to model. Future research on how to detect this correctly.
        \end{itemize}
    \fi
    
    \begin{figure}
        \centering
        \includegraphics[width=0.7\textwidth]{figures/inst_11_curves.png}
        \caption{The global model validation curves for all considered sub-compartments, of a site with problematic annotations (Institution 11). The instability in these curves could be caused by errors in annotation for the validation data (similar to errors that were observed for a small shared sample of data from this site).}
        \label{fig:problematic_convergence}
    \end{figure}
    
    
 \subsection*{FL benefits the more challenging/complicated tasks}
   
    
        \begin{figure}
      \centering
      \includegraphics[width=0.75\textwidth]{figures/dice_better_on_larger_regions.png}
      \caption{Global model's average \textit{DICE} across validation cases of participating sites across training rounds showing that the score is greater for regions with larger volumes (shading indicates 95\% confidence intervals over cases).}
      \label{fig:dice_across_regions}
   \end{figure}
   
       \iffalse
    \begin{itemize}
        \item As expected, WT is easier to segment than TC, which is easier to segment than ET (See the relative performance indicated by the curves in Fig.~\ref{dice_across_regions})
        \item Clinically actionable regions are WT and TC, and TC improves significantly
        \begin{figure}
          \centering
          \includegraphics[width=0.9\textwidth]{figures/dice_better_on_larger_regions.png}
          \caption{Global model validation \textit{DICE} over rounds showing that the score is greater for larger sized regions (shading indicates 95\% confidence intervals over cases).}
          \label{dice_across_regions}
       \end{figure}
       \item The benefits of federation are more pronounced for the more difficult segmentation sub-tasks (See ET and TC improvements compared to WT improvements in Fig.~\ref{benefits_of_fed}). We are glad to see improvement in the harder sub-tasks, rather than FL simply boosting performance on the already easy task (e.g. threshold check on the flair modality for WT segmentation).
        \item show number of collaborators where WT is on top, TC is on top and ET is on top (see Table \ref{metric_to_insts_with_it_on_top}).
        
        \begin{table}
        \centering
        \caption{List of institutions whose validation scores of the consensus model is highest in each respective metric.}
        \label{metric_to_insts_with_it_on_top}
        \begin{tabular}{lll}
        \toprule
        Metric name & Institution count & Institution names \\
        \midrule
        binary\_DICE\_ET & 4 & ['institution\_11', 'institution\_24', 'institution\_4', 'institution\_45'] \\
        binary\_DICE\_TC & 10 & ['institution\_1', 'institution\_14', 'institution\_15', 'institution\_22', 'institution\_25',\\
         & & 'institution\_26', 'institution\_33', 'institution\_40', 'institution\_44', 'institution\_8'] \\
        binary\_DICE\_WT & 34 & ['institution\_10', 'institution\_12', 'institution\_13', 'institution\_16', 'institution\_17',\\ 
        & & 'institution\_18', 'institution\_19', 'institution\_2', 'institution\_20', 'institution\_21',\\ 
        & & 'institution\_23', 'institution\_27', 'institution\_28', 'institution\_29', 'institution\_3',\\ 
        & & 'institution\_30', 'institution\_31', 'institution\_32', 'institution\_34', 'institution\_35',\\ 
        & & 'institution\_36', 'institution\_37', 'institution\_38', 'institution\_39', 'institution\_41',\\ 
        & & 'institution\_42', 'institution\_43', 'institution\_46', 'institution\_47', 'institution\_48',\\ 
        & & 'institution\_49', 'institution\_5', 'institution\_7', 'institution\_9'] \\
        \bottomrule
        \end{tabular}
        \end{table}
    \end{itemize}
    
    \begin{itemize}
        \item Global model scores for all collabs' val data
    \end{itemize}
    \fi
        \iffalse
    \begin{table}[]
    \fxwarning{SP: I don't think this table is informative enough; either we need to add more information or remove it entirely.}
    \centering
    \caption{List of institutions whose validation scores of the consensus model is highest in each respective metric.}
    \label{tab:metric_to_insts_with_it_on_top}
    \begin{tabular}{|c|c|c|}
    \hline
    \textbf{Binary DICE}           & \textbf{Number of Sites} & \textbf{Site IDs}                             \\ \hline
    ET & 4                                                          & 4, 11, 24, 45                        \\ \hline
    TC & 10                                                         & 1, 8, 14, 15, 22, 25, 26, 33, 40, 44 \\ \hline
    WT &
      34 &
      \begin{tabular}[c]{@{}c@{}}2, 3, 5, 7, 9, 10, 12, 13, \\ 16, 17, 18, 19,  20, 21, \\ 23, 27, 28, 29, 30, 31, \\ 32, 34, 35, 36, 37, 38, 39, \\ 41, 42, 43, 46, 47, 48, 49\end{tabular} \\ \hline
    \end{tabular}
    \end{table}
    \fi
    
    
    \subsection*{Optimal model selection is non-trivial}
%\subsection{Selecting optimal models separately for each region slightly outperforms a single model jointly optimized across all three}
% SP on 2022/01/31: needed to reduce char count of subheadings <40 per nature format
\label{findings:singlet_triplet}

    \iffalse
    \begin{itemize}
        \item There can be two definitions of what would constitute the ``best'' model:
            \begin{enumerate}
                \item A single model (which we call a `singlet') that performs the best average \textit{DICE} across all 3 regions in question
                \item A set of three models (which we call a `triplet') where each model performs the best for a single region. When using this triplet for inference, the final output to predict each individual region is produced using the corresponding model optimized for that region. 
            \end{enumerate}
        \item Performance analysis on unseen/out-of-sample data
            \begin{itemize}
                \item Consensus model results against hold-out data (See Fig.~\ref{all_consensus_against_holdout} and Fig.~\ref{singlet_an d_triplet_consensus_against_holdout})Here we see similar performance gains to that seen for the validation results on the one singlet consensus model already considered in Fig.~\ref{benefits_of_fed}: Data collected from: https://upenn.app.box.com/folder/143693813302?s=b1urkxx5b33wr0gazlipnspzj56jxgda
                
                \item Performance analysis of the the series of best ``singlet'' and ``triplet'' models for collaborators that never participated in the training process, so the data is completely out-of-sample.
                \item Comparisons with nnunet/deepscan/deepmedic would (most likely) result in nnunet/deepscan performing better, which is likely because either both or one of these models was used to create the ground truth annotation(s)
                \item if the ground truth was created using a method that under-segmented each region, and then annotators delineated the boundary regions, the final GT would be closer to ``gold standard'' (see \ref{nnunet_and_consensus_against_holdout})
                \item for ideal gold standard GT creation, multiple annotators should delineate the boundaries of the regions of interest and a majority voting done for each voxel under consideration
                \item Model ensemble trained using data from sites with the largest patient cohorts (UPenn, Heidelberg, UCSF and Symbiosis) comes close to performance of a fully federated model
            \end{itemize}
    \end{itemize}
    \fi
       \iffalse
   We have also done a performance comparison of the final consensus model against one of the widely-known BraTS winning methods, the nnU-Net \cite{isensee2021nnu}, and the results have been encapsulated in Fig.~\ref{fig:nnunet_and_consensus_against_holdout}. The fact that nnU-Net outperforms the final consensus model is not surprising however, as segmentation with nnU-Net is one of the automated methods used to create the baseline annotation by our tool (see Section.~\ref{methods:data} for details), which creates a significant bias of the final ground truth towards the methods used.
   \fi
   
      \iffalse
   %This figure could be used to show that the level of corrections form annotators was not so majorly deviating from the automated GT labels
   \begin{figure}
       \centering
       \includegraphics[width=0.75\textwidth]{figures/brats_and_consensus_model_scores_against_holdout.png}
        
       \caption{Scores against the full set of out-of-sample data of nnU-Net versus the singlet consensus model. Statistics are gathered over validation cases, and whiskers are given as one and a half of the inter-quartile range past the low and high quartiles.}
       \label{fig:nnunet_and_consensus_against_holdout}
       
   \end{figure}
   \fi
   
   
   
   \subsection{Availability of consensus model for clinical and low-resource environments (MOVE TO DISCUSSION? REMOVE? either way, go over plots to align with others include AVE)}



    \iffalse
    \begin{itemize}
        \item Post-training run-time optimization of model
        \item Enables computation in low-resource environments
        \item Compare consensus model with hold out data in terms of performance
    \end{itemize}

    
    \fxnote{Discussion with SB on 2021/11/30}
    Showcase 2 major findings:
    \begin{itemize}
        \item Currently model needs a GPU (or DL acceleration cards) to be run in a reasonable time frame
        \item Raw PT model needs X hours to run on a consumer class CPU, and the OV optimized model runs in X minutes to run on a consumer class CPU
    \end{itemize}
    
    \fi
    
      
   \iffalse
   \fxfatal{For Deepthi: Do we have any measurements for the memory usage improvements? If they are something we could report on, we could add it as a subfigure in Fig.~\ref{fig:ov_speedups}}
    
    \begin{table}[t]
    \centering
    \caption{Hardware configuration used for the performance tests.}
    \fxnote{This could be moved to supplementary}
    \label{Tab:hwconfig}
    \begin{tabular}{|c|c|}
    \hline
    Platform                                  & Tiger Lake                                               \\ \hline
    CPU Model                                 & Core(\texttrademark) i7-1185G7E @ 2.80GHz \\ \hline
    \# of Nodes, \# of Sockets                & 1                                                        \\ \hline
    Cores per Socket                          & 4                                                        \\ \hline
    Threads per Socket                        & 8                                                        \\ \hline
    Memory Configuration (type, slots, speed) & DDR4, 2, 3200 MT/s                                       \\ \hline
    Advanced technologies                      & AVX2, AVX512, DL Boost (VNNI)                            \\ \hline
    TDP                                       & 28W                                                      \\ \hline
    \end{tabular}
    \end{table}
    
    \fi
    
    
    
    
        \begin{figure}
        \centering
        \includegraphics[width=0.45\textwidth]{figures/singlet_versus_triplet_increases_against_holdout_V1.png}
        \caption{Percentage increases in mean (over cases) $DSC$ scores for \textit{singlet} versus \textit{triplet} consensus models over the public initial model, for the out-of-sample dataset. Statistics are gathered over instances of each model type, with whiskers given as one and a half of the inter-quartile range past the low and high quartiles.}
        \label{fig:singlet_triplet_consensus_against_holdout}
    \end{figure}
    
    
    
    \subsection*{Model Deployment in Low-Resource Settings}

    
    To facilitate use in low-resource environments, we have performed post-training run-time optimization of the consensus model (see Section.~\ref{methods:optimization} for details). As evidenced in Fig.~\ref{fig:ov_acc}, the optimized consensus model shows no significant difference in performance when evaluated against the centralized out-of-sample dataset. Such optimizations making the model viable for use in environments without dedicated hardware to accelerate DL computations. Additionally, we leverage low precision quantization to boost performance and make use of benefits from features such as the Vector Neural Network Instructions (VNNI)\footnote{\url{https://en.wikichip.org/wiki/x86/avx512_vnni}} \cite{rodriguez2018lower}. This enables the model to be inferred on cases without the use of any specialized hardware (i.e., a consumer class CPU on a laptop), thereby further magnifying the impact of the study to real-world environments. %An additional benefit of the optimization step is its run-time improvement, which is illustrated by Fig.~\ref{fig:ov_speedups}. We report the inference time performance for three configuration - in the out of box native framework (PyTorch) format (Baseline configuration), with OpenVINO optimizations for single precision format (OpenVINO FP32), and with additional low precision inference optimizations (OpenVINO INT8). We observe a total of $4.48$ times speedup in runtime performance with these optimizations compared to the baseline configuration.
    
    \begin{figure}
       \centering
       \includegraphics[width=0.75\textwidth]{figures/ov_acc_plot.png}
       \caption{Metric scores for different framework configurations the centralized out-of-sample dataset measured on Intel\textsuperscript{\textregistered} Core\textsuperscript{\texttrademark} i7-1185G7E}
       \label{fig:ov_acc}
   \end{figure}
    \begin{figure}
       \centering
       \includegraphics[width=0.75\textwidth]{figures/ov_speedup_plot.pdf}
       \caption{Improvement in inference time performance with model optimizations measured on Intel\textsuperscript{\textregistered} Core\textsuperscript{\texttrademark} i7-1185G7E}
       \label{fig:ov_speedups}
   \end{figure}
   
   
   
\subsection*{Collaborators' Perspective}
   The results of the survey are provided in Table \ref{table:collaborator_survey}.
    
    \begin{table}[]
        \centering
        \begin{tabular}{|c|c|}
        \hline
            Percent Agree & Statement  \\
            \hline
            $96\%$ & "I approve of the documentation provided regarding preprocessing and data curation." \\
            $84\%$ & "I would use the FeTS tool for my own projects or data analysis pipelines." \\
            $82.4\%$ & "I would use and recommend the automated tumor segmentation pipeline available through the FeTS tool." \\
            $86\%$ & "I used either FeTS or CaPTk or ITK-SNAP for annotation correction." \\
            $92\%$ & "I found the instructions provided for generating the secure client-side keys easy to follow." \\
            $100\%$ & "I found the instructions to start federated training easy to follow." \\
            $88\%$ & "I used a dedicated machine for my workload." \\
            $14\%$ & "I used 3D-Slicer or something other than FeTS, CaPTk or ITK-SNAP for annotation correction." \\
            $0\%$ & "I ran into an issue during preprocessing and data curation." \\
            $12\%$ & "I used a Container or virtual machine for my workload." \\
            \hline
        \end{tabular}
        \caption{Survey results for participants of the FeTS training.}
        \label{table:collaborator_survey}
    \end{table}
    
    
    
    %\subsection*{FL is robust to some annotation errors}
%consider tab:metric_to_insts_with_it_on_top (in "of no use"-results for supplementary

%\subsection*{Optimal model selection is non-trivial}
% Comparisons with nnunet/deepscan/deepmedic would (most likely) result in nnunet/deepscan performing better, which is likely because either both or one of these models was used to create the ground truth annotation(s)
% if the ground truth was created using a method that under-segmented each region, and then annotators delineated the boundary regions, the final GT would be closer to ``gold standard'' (see \ref{nnunet_and_consensus_against_holdout})
% for ideal gold standard GT creation, multiple annotators should delineate the boundaries of the regions of interest and a majority voting done for each voxel under consideration
                %results and more elaboration are included in the of no use folder.
                
                
                
                \iffalse
\subsection*{Model Deployment in Low-Resource Settings}
    To facilitate use in low-resource environments, we have performed post-training run-time optimization of the consensus model (see Section.~\ref{methods:optimization} for details). As evidenced in Fig.~\ref{fig:ov_acc}, the optimized consensus model shows no significant difference in performance when evaluated against the centralized out-of-sample dataset. Such optimizations making the model viable for use in environments without dedicated hardware to accelerate DL computations. Additionally, we leverage low precision quantization to boost performance and make use of benefits from features such as the Vector Neural Network Instructions (VNNI)\footnote{\url{https://en.wikichip.org/wiki/x86/avx512_vnni}} \cite{rodriguez2018lower}. This enables the model to be inferred on cases without the use of any specialized hardware (i.e., a consumer class CPU on a laptop), thereby further magnifying the impact of the study to real-world environments. %An additional benefit of the optimization step is its run-time improvement, which is illustrated by Fig.~\ref{fig:ov_speedups}. We report the inference time performance for three configuration - in the out of box native framework (PyTorch) format (Baseline configuration), with OpenVINO optimizations for single precision format (OpenVINO FP32), and with additional low precision inference optimizations (OpenVINO INT8). We observe a total of $4.48$ times speedup in runtime performance with these optimizations compared to the baseline configuration.
\fi





\iffalse    
\subsection*{Governing a multi-national federation}
\fxwarning{Perhaps this entire section can go in discussion?}

    A substantial amount of coordination is required to set up a multi-national real-world federation. As this study is the first at this scale and task complexity, we have compiled a set of governance insights from our experience that can serve as considerations for future successful FL studies. These insights differ from previous literature that describe studies that were smaller in scale and involved simpler tasks \cite{roth2020federated,dayan2021federated}. By governance of the federation we refer both to the accurate definition of the problem statement (including reference labels and harmonization considerations accounting for inter-site variability), and the coordination with the collaborating sites for eligibility and compliance with the problem statement definition, as well as security and technical considerations.

    The coordination began with the security teams of collaborating sites, and giving them access to the source code of the platform developed to facilitate this study. These security discussions highlighted the benefit of the platform being open-source, making security code reviews easier. Resource gathering was then carried out by identifying technical leads and assessing computational resources at each site. With the technical leads, we then proceeded to test the complete workflow to further identify gaps in the requirements, such as network configurations and hardware requirements. We then proceeded with data curation and preprocessing, % (see Section~\ref{methods:dataPreProc}), 
    and finally connected individual sites to the aggregation server to initiate their participation.

    Following the precise definition of our problem statement \cite{brats_1,brats_2,brats_3,brats_4}, ensuring strict compliance with the preprocessing and annotation protocol for the generation of reference standards was vital for the model to learn correct information during training. To this end, we instituted an extensively and comprehensively documented annotation protocol with visual example representations and common expected errors (as observed in the literature \cite{rudie2019multi,brats_4}) to all collaborators. We have further circulated an end-to-end platform developed to facilitate this federation, providing to each collaborating site all the necessary functionalities to i) uniformly curate their data and account for inter-site acquisition variability, ii) generate the reference standard labels, and iii) participate in the federated training process. % (for more details see Section methods:federation X). 
    Finally, we held interactive sessions to complement the theoretical definition of the reference standards, and further guide collaborating sites.

    In general, debugging issues with the collected data and annotations is more difficult during FL due to the level of coordination and/or privacy issues involved, since the data are always retained at the collaborating site. We gained substantial experience during this effort that went into further development of use-inspired but generalizable data sanity checking functionality in the tools we developed, towards facilitating multi-site collaborations.
    

\subsection*{Collaborators' Perspective}
\fxwarning{Perhaps this entire section can go in discussion?}
% Flinders abstract: https://www.dropbox.com/s/4k8qibr85bvflrk/FeTS_RANZCR_MST_UPenn.doc?dl=0

    Upon conclusion of the study, sites participating in the model training process were given a survey to fill in regarding various aspects of their experience. According to the provided feedback, $96\%$ of the sites found the comprehensive documentation on preprocessing and data curation essential, and thought that lack of such documentation could have resulted in inconsistent annotations. Additionally, $92\%$ found the documentation relating to establishing secure connectivity to the aggregation server easy to follow and essential to expedite reviews by the related groups. Furthermore, $84\%$ of the sites appreciated the user-friendly interface of the provided tool and its associated complete functionality (beyond its FL backend), and indicated their intention to use it and recommend it for projects and data analysis pipelines beyond the scope of this study. To generate the reference standard labels for their local data, $86\%$ of the collaborating sites indicated that they used either FeTS (i.e., the tool developed for this study), CaPTk \cite{captk_1}, or ITK-SNAP \cite{py06nimg}, whereas the remaining $14\%$ used either 3D-Slicer \cite{kikinis20143d}, the BraTS toolkit \cite{kofler2020brats}, or something else. In terms of hardware requirements at each site, $88\%$ used a dedicated workstation for their local workload, and the remaining $12\%$ used either a containerized form of the FeTS platform, or a virtual machine.

\fi

==> of no use/INTRO_draft_notes.tex <==
\iffalse
\begin{itemize}
    \item machine learning for current studies and how fl fits into it
        \begin{itemize}
            \item ML requires a \textbf{lot} of data \cite{marcus2018deep,aggarwal2018neural}
            \item ML models trained on data from a single institution can never generalize nor obtain appropriate amount of accuracy on data from unseen institutions \cite{armato2004lung,thompson2014enigma,chand2019t195,bakas2020iglass,davatzikos2020ai,habes2021brain}
            \item Solving this requires training ML model(s) from as many acquisition sites as possible \cite{armato2004lung,thompson2014enigma,chand2019t195,bakas2020iglass,davatzikos2020ai,habes2021brain}
            \item Current paradigm for doing this is by pooling data from clinical entities in a single location and then doing training \cite{armato2004lung,thompson2014enigma,chand2019t195,bakas2020iglass,davatzikos2020ai,habes2021brain} - this cannot scale when looking at sites from multiple countries with various concerns related to regulatory, cultural, IP-sharing
            \item FL aims to solve this by alleviating the need for data sharing altogether, instead only sharing the insights garnered from the data, i.e., the ML model itself \cite{mcmahan2017communication,roy2019braintorrent,sheller2020federated,rieke2020future,kaissis2020secure,dayan2021federated}
            \item FL performs similarly to centralized learning \cite{chang2018distributed,nilsson2018performance,wang2019adaptive,sheller2020federated,sarma2021federated} [ref: EXAM paper??? did this talk about centralized comparison? \fxnote{For Spyros: which paper is this? If you are referring to NVIDIA's Nat Med paper, they did not talk about federated/centralized difference}, other papers showing parity in medical use cases between FL and centralized training]
            \item when done across multiple sites, models trained using FL can obtain similar performance as compared to those trained using pooled data \cite{sheller2020federated}
            \item this has also been shown by real-world studies \cite{shen2021multi,yang2021federated,flores2021federated} (refer to the 2-3 cases of individual 5-collab papers)
        \end{itemize}
    \item Why to leverage this for glioblastoma (GBM)
        \begin{itemize}
            \item GBMs are highly heterogeneous in nature \cite{pati2020reproducibility,ostrom2019cbtrus}, and data from different sites tend to have extremely varying characteristics \cite{chaichana2013multi,fathi2020cancer}
            \item It is very rare disease, which doesn't let a single institution reach ``critical mass'' in terms of the number of cases needed to train a robust DL model
            \item the most important regions of GBM are ET, TC, WT - give detailed explanation of the regions, along with illustration; give description of NCR and ED 
            \item delineating these regions \cite{brats_1,brats_2,brats_3,brats_4} is a critical first step towards further clinical analyses such as survival \cite{brats_3,fathi2020cancer,bakas2020overall,nicolasjilwan2015addition,prasanna2017radiomic} and recurrence predictions \cite{fathi2020cancer,han2018patient,akbari2016imaging,shukla2017advanced,chang2016multimodal}
            \item BraTS challenge \cite{brats_1,brats_2,brats_3,brats_4} has been instrumental in ensuring the presence of a large and diverse data cohort, and this has pushed the envelope for GBM segmentation to new frontiers
            \item However large the challenge cohort becomes, it still fails to address the inherent complexity and heterogeneity of the pathology in question, which necessitates the participation of multiple clinical partners to provide data
            \item instead of going through multiple regulatory channels, we addressed this problem using FL
        \end{itemize}
    \item More details on current state-of-the-art for FL
        \begin{itemize}
            \item Previous Scientific reports study
            \item Briefly summarize the NV's nature medicine paper
            \item Succinctly differentiate how our study from previous studies: key question and difference is use of data annotated at each edge by clinical experts following a specific schema.
        \end{itemize}
    \item Brief overview of what we have done in this study
        \begin{itemize}
            \item Started with a baseline neural network to finalize the data science algorithm that can perform the segmentation of the aforementioned regions
            \item ``Data science algorithm'' is defined as all the steps required to process a dataset, starting with preprocessing and ending with model training (and post-processing, if applicable) \cite{kotu2018data}
            \item We federated the established data science algorithm using completely open-sourced tools to encourage  findability, accessibility, interoperability, and reusability (FAIR) in scientific research \cite{wilkinson2016fair}
            \item We developed and deployed a tool that performs end-to-end processing of the data along with the deep learning based training to more than $n=60$ clinical sites, by taking extreme care of necessary info-sec requirements
        \end{itemize}
\end{itemize}
\fi


Prior simulated and real-world studies have shown that when multiple sites are contributing data, models trained using FL perform similarly to those trained using CL \cite{chang2018distributed,nilsson2018performance,sheller2018multiinstitutional,wang2019adaptive,sheller2020federated,sarma2021federated,shen2021multi,yang2021federated,flores2021federated}.

==> of no use/METHODS_draft_notes.tex <==

\iffalse
\begin{itemize}
    \item The data
        \begin{itemize}
            \item Acquisition details (include as many scanner variations as possible): multi-parametric magnetic resonance images (mpMRI) with 4 structural modalities: T1, T1-post contrast, T2, T2-FLAIR
            \item Data harmonization pipeline as described in BraTS \cite{brats_1,brats_2,brats_3,brats_4}
                \begin{enumerate}
                    \item \textit{DICOM conversion:} The originally acquired DICOM scans \cite{pianykh2012digital} are converted to the Neuroimaging Informatics Technology Initiative (NIfTI) file format \cite{nifti} for easier parsing during the computational process. Additionally, it has the added benefit of stripping all patient-identifiable metadata from the scans \cite{li2016first,white2020data}.
                    \item \textit{Bias Field Correction:} Taking into consideration we have previously shown that use of non-parametric, non-uniform intensity normalization (i.e., N4) to correct for intensity non-uniformities caused by the inhomogeneity of the scanner's magnetic field during image acquisition obliterates the MRI signal relating to the abnormal/tumor regions, we intentionally use N4 bias field correction in the preprocessing pipeline to facilitate a more optimal rigid registration across the difference MRI sequences.
                    \item \textit{Rigid Registration:} The bias field corrected images are registered to the T1Gd image, and the T1Gd image is rigidly registered to the SRI24 atlas \cite{sri} to obtain 2 sets of transformation matrices. These matrices are then aggregated to a single matrix which defines the transformation of each modality to the atlas, which ensures that every image has a cohesive data shape ($[240,240,155]$) and voxel resolution ($1mm^3$). We apply this aggregated matrix to the original scans (instead of the bias-corrected images) to maximize the fidelity of the image. The registration is performed using the Greedy framework\footnote{\url{https://github.com/pyushkevich/greedy}} \cite{yushkevich2016fast}  (available in the Cancer Imaging Phenomics Toolkit (CaPTk) \cite{captk_1,captk_2,captk_3}, ITK-SNAP \cite{py06nimg}, and the open-source FeTS Tool\footnote{\url{https://www.fets.ai/}}, which was provided to all collaborators for this study).
                    \item \textit{Skull Stripping:} This step involves the extraction of the brain from all co-registered scans, which ensures significantly improved performance for tumor segmentation tasks \cite{brats_1,brats_2,brats_3,brats_4}, and was performed using the Brain Mask Generator (BrainMaGe) tool\footnote{\url{https://github.com/CBICA/BrainMaGe}} \cite{thakur2020brain}, which is available through both CaPTk and the FeTS tool, and the resulting brain mask was manual revised when needed to ensure that the complete abnormal hyper-intense FLAIR signal is always included within it.
                    \item \textit{Generation of automated baseline segmentations:} To provide a reasonably good baseline, we provided segmentations from three popular methods from the BraTS challenge using their pre-trained models: i) DeepMedic \cite{kamnitsas2017efficient}, ii) DeepScan \cite{mckinley2018ensembles}, and iii) nnU-Net \cite{isensee2021nnu}. Along with segmentations from each method, we also provide labels using various fusion strategies from these methods, namely, i) standard voting \cite{rohlfing2004performance}, ii) STAPLE \cite{rohlfing2005multi}, iii) majority voting \cite{huo2015label}, and iv) selective and iterative method for performance level estimation (SIMPLE) \cite{langerak2010label}. All implementations are available through the FeTS tool via the Label Fusion package \cite{labelfusion}.
                \end{enumerate}
            \item Describe BraTS data and annotation protocol.
            \item Describe the out-of-sample datasets
        \end{itemize}
    \item The network
        \begin{itemize}
            \item We use a 3D U-Net with residual connections \cite{pati2021gandlf,thakur2020brain,ronneberger2015u,drozdzal2016importance,he2016deep,cciccek20163d,bhalerao2019brain} to segment the different regions, ET, TC, ET
            \item Illustration provided in Fig.\ref{fig:unet}
            \begin{figure}
              \centering
              \includegraphics[width=0.9\textwidth]{figures/unet.png}
              \caption{Illustration of the U-Net architecture, which was used with residual connections, plotted using PlotNeuralNet \cite{iqbal2018harisiqbal88}.}
              \label{fig:unet}
           \end{figure}
            \item The network had $n=30$ base filters, with a minimum and maximum learning rate of $lr=0.00005$ which cycles at the rate of $n=2$ epochs, which was optimized using the Adam optimizer \cite{kingma2014adam}. We used the generalized \textit{DICE} score \cite{dice} as the loss function \cite{sudre2017generalised}, but instead of using the regions themselves, we used the mirrored variant, which has been shown to capture variations in smaller regions better \cite{isensee2021nnu}, which did not require us to use penalties in the loss function \cite{chen2016efficient,salehi2017tversky,caliva2019distance}. The final layer of the model was a sigmoid layer, since we wanted to ensure that region overlap was properly taken into account during model training and inference.
            \item Describe the difference between binary and floating dice
        \end{itemize}
    \item Data loading and handling % (\label{methods:data_processing})
        \begin{itemize}
            \item We leveraged the data loading logic from GaNDLF \cite{pati2021gandlf} to ensure we are able to experiment with various data augmentation techniques
            \item For preprocessing, we removed the all-zero axial planes from the images, and performed a z-score normalize of the non-zero image intensities \cite{reinhold2019evaluating}
            \item We performed patch-based training, and kept the patch size constant at $128 \times 128 \times 128$ to ensure that we are able to fit the model to the base hardware that was available with collaborators (a discrete GPU with \textit{at least} 11GB of dedicated VRAM), and we extracted a single patch per volume during every epoch
            \item All of them were
            \item For data augmentation, we leveraged TorchIO \cite{garcia_torchio_2020} in combination with GaNDLF \cite{pati2021gandlf}. Specifically, we used the following:
                \begin{enumerate}
                    \item random noise augmentation with mean of $m=0.0$, standard deviation of $std=0.1$ with probability of $p=0.2$
                    \item random Rotation augmentations of both $90^\circ$ and $180^\circ$, each along all the axes and with probability of $p=0.5$
                    \item random flip augmentation for all axes with probability of $p=1.0$
                \end{enumerate}
        \end{itemize}
    \item The federation
        \begin{itemize}
            \item Use figure for federation
            \item The map Fig.~\ref{fig:map}
            
                \begin{figure}
                    \centering
                    \includegraphics[width=1.0\textwidth]{figures/map.png}
                    \caption{The map of all FeTS collaborators, showcasing the truly global footprint.}
                    \label{fig:map}
                \end{figure}
                
            \item Collaborators train the same data science algorithm on their own data and share the model updates with a central aggregator
            \item The central aggregator node receives the model updates, combines them from all collaborators and send the consensus model back.
            \item This process is repeated till model converges
            \item Perhaps talk about SGX and TEE here? \fxnote{For Brandon to expand on}
            \item Talk about the ``initial'' or ``baseline'' model, which is trained on the BraTS 2020 subjects after removing data from the sites that participate in the federation
        \end{itemize}
    \item Model Optimization
        \item \fxnote{For Deepthi to fill}
        \item Clinical environments typically have constraints in compute resources such as the availability of compute and memory. Performance of deep Learning workloads such as the consensus model inference could suffer under such limitations.  
        \item The goal is to optimize these workloads under these constraints by leveraging optimization toolkits such as OpenVINO\footnote{\url{https://docs.openvino.ai/latest/index.html}} \cite{gorbachev2019openvino}. 
        %Intel OpenVINO is a toolkit that enables acceleration of neural network models through various optimizations such as operators fusion, stride optimizations, etc.
        \item In addition to training the most comprehensive DL model for brain tumor segmentation, we have explored leveraging the OpenVINO toolkit for its post-training optimization for low precision inference.
        \item We make use of optimizations such as operators fusion, stride optimizations through the OpenVINO toolkit.
        \item Low precision inference provides performance benefits such as lower inference latency and higher throughput. The trade-off would be a small drop in the model accuracy. We present results from the low precision optimizations for the consensus model.
        \item Our model optimization methodology is as follows: We first obtained the consensus model which was is a PyTorch native framework format. We use the OpenVINO model optimizer to convert the model to an intermediate representation format.
        Additionally we convert the floating point single precision model to a fixed precision 8-bit integer model through a process known as quantization. In particular, we use accuracy aware quantization method where the layers in the models are iteratively scaled to the lower precision format.
        
        
        %
        \item Maybe include model deployment, if appropriate?
\end{itemize}
\fi

\iffalse
\subsection*{Data/Code availability}

    \begin{itemize}
        \item Additional functionality based on CaPTk [REFS], such as population-based harmonized preprocessing, DCM2NII conversion, coregistration, manual refinements
        \item SRI
        \item BrainMaGE
        \item dockers of nnunet, deepscan, deepmedic
        \item FL backend developed for this project has been open-sourced to encourage further research on FL as part of collaboration with Intel [REF-OpenFL]
        \item Data science algorithm was developed using GaNDLF [REF]
        \item All codebase used for this project is available at \url{https://github.com/FETS-AI}
        \item TorchIO for augmentations
    \end{itemize}
\fi







%OPTIMIZATION


\iffalse
    \item Model Optimization
        \begin{itemize}
            \item Clinical environments typically have constraints in compute resources such as the availability of compute and memory. Performance of deep Learning workloads such as the consensus model inference could suffer under such limitations.  
            \item The goal is to optimize these workloads under these constraints by leveraging optimization toolkits such as OpenVINO\footnote{\url{https://docs.openvino.ai/latest/index.html}} \cite{gorbachev2019openvino}. 
            %Intel OpenVINO is a toolkit that enables acceleration of neural network models through various optimizations such as operators fusion, stride optimizations, etc.
            \item In addition to training the most comprehensive DL model for brain tumor segmentation, we have explored leveraging the OpenVINO toolkit for its post-training optimization for low precision inference.
            \item We make use of optimizations such as operators fusion, stride optimizations through the OpenVINO toolkit.
            \item Low precision inference provides performance benefits such as lower inference latency and higher throughput. The trade-off would be a small drop in the model accuracy. We present results from the low precision optimizations for the consensus model.
            \item Our model optimization methodology is as follows: We obtained the consensus model which is a PyTorch native framework format. We use the OpenVINO model optimizer to convert the model to an intermediate representation format.
            Additionally we convert the floating point single precision model to a fixed precision 8-bit integer model through a process known as quantization. In particular, we use accuracy aware quantization method where the layers in the models are iteratively scaled to the lower precision format.
        \end{itemize}

\subsection*{Model run-time}
\label{methods:optimization}
%%First paragraph establishes the problem, explains how we use a single, relatively small model, which reduces computational resource requirements. Then the second paragraph could be something like "To explore further optimizations, we applied neural network optimizations from the OpenVINO toolkit". We want the story to be "Reducing computational requirements is good. We did it with a simple non-ensemble model. We then took it another step by testing these optimizations. Check out what we found."
    In addition to training our DL model on such a comprehensive brain tumor dataset, we emphasize that our final model is a single 3D residual UNet rather than a multiple model ensemble. As such, the run time for use of our model is reduced from that of an ensemble. 
    %We have also explored how it could be used in as many scenarios as possible, especially in the clinic. Clinical environments typically have constraints in compute resources such as the availability of specialized hardware and memory. Performance of deep Learning workloads such as the consensus model inference could suffer under such limitations. The goal is to optimize the model inference workload under these constraints by leveraging optimization toolkits such as OpenVINO\footnote{\url{https://docs.openvino.ai/latest/index.html}} \cite{gorbachev2019openvino}. OpenVINO is a toolkit that enables acceleration of neural network models through various optimizations such as operators fusion. In this study, we use graph level optimizations such as operators fusion as well optimizations for low precision inference. Low precision inference provides performance benefits such as lower inference latency and higher throughput, and the trade-off is expected be a small drop in the model accuracy. We obtained the consensus model in a PyTorch native format. We use the OpenVINO model optimizer to convert the model to an intermediate representation format, following which we convert the floating point single precision model to a fixed precision 8-bit integer model through a process known as ``quantization'' \cite{lin2016fixed}. In particular, we use accuracy-aware quantization method \cite{vakili2013enhanced}, where the layers in the models are iteratively scaled to the lower precision format.
    \fi
